Ultra-Cold Cryogenic TEM with Liquid Helium and High Stability

Cryogenic transmission electron microscopy has revolutionized structural biology and materials science, but achieving temperatures below the boiling point of liquid nitrogen remains a long-standing aspiration. We introduce an ultra-cold liquid helium transmission electron microscope specimen holder, featuring continuous cryogen flow and vibration decoupling. This instrument is compatible with modern aberration-corrected microscopes and achieves sub-25 K base temperature, ${\pm}$2 mK thermal stability over many hours, and atomic resolution--setting the stage for a new era of cryogenic electron microscopy.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        #system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
